Architecture, Dataflow and Physical Design Implications of 3D-ICs for DNN-Accelerators

The everlasting demand for higher computing power for deep neural networks (DNNs) drives the development of parallel computing architectures. 3D integration, in which chips are integrated and connected vertically, can further increase performance because it introduces another level of spatial parallelism. Therefore, we analyze dataflows, performance, area, power and temperature of such 3D-DNN-accelerators. Monolithic and TSV-based stacked 3D-ICs are compared against 2D-ICs. We identify workload properties and architectural parameters for efficient 3D-ICs and achieve up to 9.14x speedup of 3D vs. 2D. We discuss area-performance trade-offs. We demonstrate applicability as the 3D-IC draws similar power as 2D-ICs and is not thermal limited.

==> data/temp/temp.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage[dvipsnames]{xcolor}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.8}
%\usepackage{amssymb}
%\usepackage{units}
%\usepackage{colortbl}
%
%\usetikzlibrary{decorations.pathreplacing, decorations, positioning, calc, patterns, arrows, math, shadings, matrix}
%\input{../../fig/defs.tex}
%
%
%\begin{document}
	\begin{tikzpicture}
		\begin{axis}[
		axis line style={lightgray},
		ymajorgrids,
%		ymax = 1.08,
%		ymin = 0.25,
%		xmin = 0,
%		xmax = 11,
%	%	ybar = 0pt,
%		title={Restnet 50},
		title style = {font =\small, yshift =-5},
		label style={font=\scriptsize},
		ylabel style = {yshift = -15},
		xlabel style = {yshift = 5},
		x tick label style={font=\scriptsize, yshift = 0},
		y tick label style = {font=\scriptsize},
		legend style = {font = \tiny},
   		legend pos = north west,
   		legend image post style={scale=0.4},
   		legend style={row sep=-4pt},
   		legend columns=3,
   		legend cell align={left},
	%	restrict y to domain*=0:1.5,
%			visualization depends on=rawy\as\rawy,
%			 after end axis/.code={ % Draw line indicating break
%				\draw [ultra thick, white, decoration={snake, amplitude=1pt}, decorate] (rel axis cs:0,1.05) -- (rel axis cs:1,1.05);
%			},
		xlabel = {},
		ylabel = {Temperature [K]},
		xtick= {1, 2, 3, 4, 5, 6},
		xticklabels = {2D-IC, {3D-IC w/TSV\\near heatsink},  {3D-IC w/TSV\\other layers},{3D-IC w/MIV\\near heatsink},  {3D-IC w/MIV\\other layers}}, 
		%symbolic x coords={1,2,3,4,5},
		height =4.1cm,
		width = 1.3\linewidth, 
		%		ymin= 0.9
	%	bar width=0.11cm,
		%every axis plot/.append style={fill,draw=none,no markers},
		ytick style={draw=none},
		xtick style={draw=none},clip=false,
		xticklabel style={align=center},	]
		%small:
		
		\draw[-, col1, very thick]  (axis cs:1, 324.3) --  (axis cs:1, 324.65);
		\draw[-, col1, very thick]  (axis cs:2, 324.47) --  (axis cs:2, 325.85);
		\draw[-, col1, very thick]  (axis cs:3, 326.13) --  (axis cs:3, 328.24);
		\draw[-, col1, very thick]  (axis cs:4, 328.09) --  (axis cs:4, 328.26);
		\draw[-, col1, very thick]  (axis cs:5, 331.81) --  (axis cs:5, 332.02);
		\addplot[col1, only marks, mark = x] table[x=id,y=smallmin, col sep=comma] {data/temp/temp.csv};\label{plot:temp:smallmin}
		\addplot[col1,  only marks,mark = x] table[x=id,y=smallmax, col sep=comma] {data/temp/temp.csv};\label{plot:temp:smallmax}
			
		
		
		%large:
		\draw[-, col2, very thick]  (axis cs:1, 327.29) -- (axis cs:1, 328.28);
		\draw[-, col2, very thick]  (axis cs:2, 326.8 ) -- (axis cs:2, 328.24);
		\draw[-, col2, very thick]  (axis cs:3, 328.1 ) -- (axis cs:3, 330.06);
		\draw[-, col2, very thick]  (axis cs:4, 330.74) -- (axis cs:4, 331.44);
		\draw[-, col2, very thick]  (axis cs:5, 334.5 ) -- (axis cs:5, 335.14);
		
		\addplot[col2, only marks,mark = x] table[x=id,y=largemin, col sep=comma] {data/temp/temp.csv};\label{plot:temp:largemin}
		\addplot[col2,  only marks,mark = x] table[x=id,y=largemax, col sep=comma] {data/temp/temp.csv};\label{plot:temp:largemax}
		
		
		

%		\draw [thick, red] ({rel axis cs:0,0}|-{axis cs:2,1}) -- ({rel axis cs:1,0}|-{axis cs:2,1}) node [pos=0.90, above] {\sffamily \scriptsize $\Uparrow$ worse} node [align = left, pos=0.15, below] {\sffamily \scriptsize $\Downarrow$ better};
%%		\legend{{MAC = 4096, K = 12100}, {MAC = 4096, K = 784}, {MAC = 4096, K = 255},
%%		{MAC = 32768, K = 12100}, {MAC = 32768, K = 784}, {MAC = 32768, K = 255},
%%		{MAC = 262144, K = 12100}, {MAC = 262144, K = 784}, {MAC = 262144, K = 255}};
	 \coordinate (legend) at (axis description cs:0.01,0.99);
		\end{axis}	
%	\matrix [
%	fill = white, 
%	draw,
%	every node/.append style={%
%		inner xsep=0pt,
%		inner ysep=0pt, 
%		draw=lightgray, % just to show node borders
%		text height=10,%\heightof{0},
%		text width=24,
%		align=center
%	},
%	matrix of nodes,
%	anchor=north west,
%	] at (legend) {
%		\tiny MAC\textbackslash K & \tiny \phantom{\textbackslash}12100 & \tiny \phantom{\textbackslash}784 & \tiny \phantom{\textbackslash}255\\
%		\tiny 4096 & \scalebox{1.5}{\ref{plot:2:line1}} & \scalebox{1.5}{\ref{plot:2:line2}} & \scalebox{1.5}{\ref{plot:2:line3}}   \\
%		\tiny 32768 & \scalebox{1.5}{\ref{plot:2:line21}} & \scalebox{1.5}{\ref{plot:2:line22}} & \scalebox{1.5}{\ref{plot:2:line23}}   \\
%		\tiny 262144 & \scalebox{1.5}{\ref{plot:2:line31}} & \scalebox{1.5}{\ref{plot:2:line32}} & \scalebox{1.5}{\ref{plot:2:line33}}   \\
%	};

	\node [anchor = north west ]at (legend) {
\begin{tabular}{|c|c|}

\hline 	
\cellcolor{white} 3 Layers @ 16000 MACs&\cellcolor{white}\ref{plot:temp:smallmin}\\
\hline 
\cellcolor{white} 3 Layers @ 64000 MACs&\cellcolor{white}\ref{plot:temp:largemin}\\
\hline
  \end{tabular} 	
};

	\end{tikzpicture}
	
			
%\end{document}


==> fig/dataflow/IS_df.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.8}
%\usepackage{amssymb}
%\usepackage{units}
%\usetikzlibrary{decorations.pathreplacing, decorations, positioning, calc, patterns, arrows, math, shadings}
%\input{../defs.tex}
%
%\begin{document}
\begin{tikzpicture}[scale = .3, yscale = -1]


%systolic array
\draw[fill = lightgray!50] (-.5, -.5) rectangle (11,6);
%PEs
\foreach \x in {0,1,...,10}{
	\foreach \y in {0,1,...,5}{
		\draw[fill = white, rounded corners = 0.75](\x,\y) rectangle ++(.5,.5);
	}
}

%upper matrix
\draw[draw= cInput, fill = cInput!80] (0,-1) rectangle ++ (10.5,-4) node [midway, white] {IFMAP};
\draw[latex-latex] (0,-5.5) -- ++(10.5,0) node [midway, above] {$S_C$};
\draw[latex-latex] (-.5,-1) -- ++(0,-4) node [midway, left] {$S_R$};

%left matrix
\draw[draw = cFilter, fill = cFilter!80] (-1,0) rectangle ++ (-4, 5.5)  node [midway, white] {Filter};
\draw[latex - latex] (-1,-.5) -- ++(-4, 0) node [midway, above] {$T$};
\draw[latex - latex] (-5.5, 0) -- ++ (0,5.5) node[midway, left] {$S_R$};

%bottom matrix
\draw[draw = cOutput, fill = cOutput!80] (0, 6.5) rectangle ++ (10.5, 5.5)  node [midway, white] {OFMAP};
\draw[latex - latex] (-.5, 6.5) -- ++ (0,5.5) node [midway, left] {$T$};
\draw[latex - latex] (0, 12.5) -- ++ (10.5, 0) node [midway, below] {$S_C$};

%data movement arrows
%\draw[- latex, very thick, cFilter] (-2, 5.75) -- ++ (3,0);
%\draw[- latex, very thick, cInput] (10.75, -2) -- ++ (0, 3);
%\draw[- latex, very thick, cOutput] (10.75, 4.5) -- ++ (0, 3);
\draw[- latex, very thick, cFilter] (-1, 2.75) -- ++ (3,0);
\draw[- latex, very thick, cInput] (5.25, -1) -- ++ (0, 3);
\draw[- latex, very thick, cOutput] (5.25, 3.5) -- ++ (0, 3);

\end{tikzpicture}

%\end{document}

==> fig/dataflow/OS_df.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.8}
%\usepackage{amssymb}
%\usepackage{units}
%\usetikzlibrary{decorations.pathreplacing, decorations, positioning, calc, patterns, arrows, math, shadings}
%\input{../defs.tex}
%
%\begin{document}
\begin{tikzpicture}[scale = .3, yscale = -1]


%systolic array
\draw[fill = lightgray!50] (-.5, -.5) rectangle (11,6);
%PEs
\foreach \x in {0,1,...,10}{
	\foreach \y in {0,1,...,5}{
		\draw[fill = white, rounded corners = 0.75](\x,\y) rectangle ++(.5,.5);
	}
}

%upper matrix
\draw[draw= cFilter, fill = cFilter!80] (0,-1) rectangle ++ (10.5,-4) node [midway, white] {Filter};
\draw[latex-latex] (0,-5.5) -- ++(10.5,0) node [midway, above] {$S_C$};
\draw[latex-latex] (-.5,-1) -- ++(0,-4) node [midway, left] {$T$};

%left matrix
\draw[draw = cInput, fill = cInput!80] (-1,0) rectangle ++ (-4, 5.5)  node [midway, white] {IFMAP};
\draw[latex - latex] (-1,-.5) -- ++(-4, 0) node [midway, above] {$T$};
\draw[latex - latex] (-5.5, 0) -- ++ (0,5.5) node[midway, left] {$S_R$};

%bottom matrix
\draw[draw = cOutput, fill = cOutput!80] (0, 6.5) rectangle ++ (10.5, 5.5)  node [midway, white] {OFMAP};
\draw[latex - latex] (-.5, 6.5) -- ++ (0,5.5) node [midway, left] {$S_R$};
\draw[latex - latex] (0, 12.5) -- ++ (10.5, 0) node [midway, below] {$S_C$};

%data movement arrows
%\draw[- latex, very thick, cInput] (-2, 5.75) -- ++ (3,0);
%\draw[- latex, very thick, cFilter] (10.75, -2) -- ++ (0, 3);
%\draw[- latex, very thick, cOutput] (10.75, 4.5) -- ++ (0, 3);
\draw[- latex, very thick, cInput] (-1, 2.75) -- ++ (3,0);
\draw[- latex, very thick, cFilter] (5.25, -1) -- ++ (0, 3);
\draw[- latex, very thick, cOutput] (5.25, 3.5) -- ++ (0, 3);

\end{tikzpicture}

%\end{document}


==> fig/dataflow/WS_df.tex <==
%\documentclass[border=2mm]{standalone}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.8}
%\usepackage{amssymb}
%\usepackage{units}
%\usetikzlibrary{decorations.pathreplacing, decorations, positioning, calc, patterns, arrows, math, shadings}
%\input{../defs.tex}
%
%\begin{document}
\begin{tikzpicture}[scale = .3, yscale = -1]


%systolic array
\draw[fill = lightgray!50] (-.5, -.5) rectangle (11,6);
%PEs
\foreach \x in {0,1,...,10}{
	\foreach \y in {0,1,...,5}{
		\draw[fill = white, rounded corners = 0.75](\x,\y) rectangle ++(.5,.5);
	}
}

%upper matrix
\draw[draw= cFilter, fill = cFilter!80] (0,-1) rectangle ++ (10.5,-4) node [midway, white] {Filter};
\draw[latex-latex] (0,-5.5) -- ++(10.5,0) node [midway, above] {$S_C$};
\draw[latex-latex] (-.5,-1) -- ++(0,-4) node [midway, left] {$S_R$};

%left matrix
\draw[draw = cInput, fill = cInput!80] (-1,0) rectangle ++ (-4, 5.5)  node [midway, white] {IFMAP};
\draw[latex - latex] (-1,-.5) -- ++(-4, 0) node [midway, above] {$T$};
\draw[latex - latex] (-5.5, 0) -- ++ (0,5.5) node[midway, left] {$S_R$};

%bottom matrix
\draw[draw = cOutput, fill = cOutput!80] (0, 6.5) rectangle ++ (10.5, 5.5)  node [midway, white] {OFMAP};
\draw[latex - latex] (-.5, 6.5) -- ++ (0,5.5) node [midway, left] {$T$};
\draw[latex - latex] (0, 12.5) -- ++ (10.5, 0) node [midway, below] {$S_C$};

%data movement arrows
%\draw[- latex, very thick, cInput] (-2, 5.75) -- ++ (3,0);
%\draw[- latex, very thick, cFilter] (10.75, -2) -- ++ (0, 3);
%\draw[- latex, very thick, cOutput] (10.75, 4.5) -- ++ (0, 3);
\draw[- latex, very thick, cInput] (-1, 2.75) -- ++ (3,0);
\draw[- latex, very thick, cFilter] (5.25, -1) -- ++ (0, 3);
\draw[- latex, very thick, cOutput] (5.25, 3.5) -- ++ (0, 3);

\end{tikzpicture}

%\end{document}

==> packages.tex <==
% Packages from the IEEE conf fromat

\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}

% Anand added
\usepackage{mathtools}
\usepackage{algorithm2e}
\usepackage{comment}

% Imported packages 
\usepackage{hyperref}

\usepackage{subcaption}

\usepackage[dvipsnames]{xcolor}
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing, decorations, decorations.pathmorphing}
\input{figs/defs}
\usepackage{pgfplots}
